A Comprehensive Performance Study of Large Language Models on Novel AI Accelerators

Artificial intelligence (AI) methods have become critical in scientific applications to help accelerate scientific discovery. Large language models (LLMs) are being considered as a promising approach to address some of the challenging problems because of their superior generalization capabilities across domains. The effectiveness of the models and the accuracy of the applications is contingent upon their efficient execution on the underlying hardware infrastructure. Specialized AI accelerator hardware systems have recently become available for accelerating AI applications. However, the comparative performance of these AI accelerators on large language models has not been previously studied. In this paper, we systematically study LLMs on multiple AI accelerators and GPUs and evaluate their performance characteristics for these models. We evaluate these systems with (i) a micro-benchmark using a core transformer block, (ii) a GPT- 2 model, and (iii) an LLM-driven science use case, GenSLM. We present our findings and analyses of the models' performance to better understand the intrinsic capabilities of AI accelerators. Furthermore, our analysis takes into account key factors such as sequence lengths, scaling behavior, sparsity, and sensitivity to gradient accumulation steps.

==> tex/02_Background.tex <==
\section{AI Accelerators}
\label{sec:accelerators}
There is also an emergence of new hardware platforms that are different from mainstream and widely used systems such as CPUs and GPUs.
%
These new accelerators  are aimed to run AI applications efficiently with novel mechanisms such as dataflow architectures and massive compute engines.
%

For this evaluation study, we used the following AI accelerators.
%
More details of these systems are listed in Table \ref{table:hwoverview}.
%
\\ \todo{add the largest model on each system to highlight their current capability}\\
\textbf{\textit{Nvidia A100:}} The A100 GPU consists of 6912 cuda cores and 432 Tensor cores to accelerate parallel workloads.
%
On a single DGX node, there are 4 A100 GPUs, interconnected with NVLink. \\
\textbf{\textit{Cerebras CS-2:}} The Cerebras CS-2 is a wafer-scale deep learning accelerator comprising 850,000 processing cores, each providing 48KB of dedicated SRAM memory for an on-chip total of 40 GB and interconnected to optimize bandwidth and latency.
%
The system has been scaled to two CS-2 wafer-scale engines nodes interconnected by the SwarmX fabric together with the MemoryX memory subsystem to enable large models.
%
Its software platform integrates popular machine learning frameworks such as TensorFlow and PyTorch. \\ 
\textbf{\textit{SambaNova SN30:}} The SambaNova DataScale system is architectured around the second-generation Reconfigurable Dataflow Unit (RDU) processor for optimal dataflow processing and acceleration.
%
The system consists of eight nodes, each of which features eight RDUs interconnected to enable model and data parallelism.
%
SambaFlow, its software stack, extracts, optimizes, and maps dataflow graphs to the RDUs from PyTorch machine learning frameworks.
%
SN30 can currently train models up to 13B parameters with a sequence length 64K on a single socket. \\ 
\textbf{\textit{Graphcore BowPod64}}: The Graphcore 22 petaflops Bow Pod64 system is the latest next-generation accelerator from Graphcore.
%
This is a one-rack system consisting of 64 Bow-class IPUs with a custom interconnect.
%
The Graphcore software stack includes support for TensorFlow and PyTorch.
%
It includes the Poplar SDK used by machine learning frameworks. \\
\textbf{\textit{Habana Gaudi2:}} The Habana Gaudi processor features eight fully programmable VLIW SIMD tensor processor cores, integrating ten 100 GbE ports of RDMA over Converged Ethernet (RoCE) into each processor chip to efficiently scale training.
%
The Gaudi system consists of two HLS-1H nodes, each with four Gaudi HL-205 cards.
%
The software stack comprises the SynapseAI stack and provides support for TensorFlow and PyTorch. \\
\textbf{\textit{AMD MI250:}} The AMD MI250 GPU is based on CDNA2 architecture, consists of 13,312 stream processors distributed across 208 compute units coupled with 128GB of dedicated HBM2e memory with 3.276TB/s of memory bandwidth.
%
It is able to achieve 362.1 TFlops of FP16 and 45.3 TFlops of FP32 peak performance.
%
Each GPU is connected to host using PCIe Gen4 and uses Infiniband for to inter-node communication. 
%
AMD ROCm open software platform support common DL stack, including Tensorflow, Pytorch in addition to libraries, such as rocBLAS, rocSPARSE, rocFFT and RCCL (ROCm Collective Communication Library) to support state-of-the-art performance in  computations and  communication on AMD GPUs. \\
\textbf{\textit{Groq GroqRack: }}A Groq Tensor Streaming Processor (TSP) provides a scalable, programmable processing core and memory building block able to achieve 250 TFlops in FP16 and 1 PetaOp/s in INT8 performance.
%
The Groq system has been recently upgraded to a GroqRack with nine Groq nodes, each consisting of eight GroqChip v1.5 Tensor streaming processors (TSP) accelerators.
%
GroqChip accelerators are interconnected via a proprietary chip-to-chip interconnect to enable larger models and data parallelism.
%
The Groq system is highly optimized for inference. \\
